Here's a Free Lunch: Sanitizing Backdoored Models with Model Merge

The democratization of pre-trained language models through open-source initiatives has rapidly advanced innovation and expanded access to cutting-edge technologies. However, this openness also brings significant security risks, including backdoor attacks, where hidden malicious behaviors are triggered by specific inputs, compromising natural language processing (NLP) system integrity and reliability. This paper suggests that merging a backdoored model with other homogeneous models can significantly remediate backdoor vulnerabilities even if such models are not entirely secure. In our experiments, we verify our hypothesis on various models (BERT-Base, RoBERTa-Large, Llama2-7B, and Mistral-7B) and datasets (SST-2, OLID, AG News, and QNLI). Compared to multiple advanced defensive approaches, our method offers an effective and efficient inference-stage defense against backdoor attacks on classification and instruction-tuned tasks without additional resources or specific knowledge. Our approach consistently outperforms recent advanced baselines, leading to an average of about 75% reduction in the attack success rate. Since model merging has been an established approach for improving model performance, the extra advantage it provides regarding defense can be seen as a cost-free bonus.

==> name.tex <==
\author{Ansh Arora $^\spadesuit$ \qquad Xuanli He$^\clubsuit$ \qquad Maximilian Mozes$^\clubsuit$ \\ \textbf{Srinibas Swain}$^\spadesuit$ \qquad \textbf{Mark Dras}$^\diamondsuit$ \qquad \textbf{Qiongkai Xu}$^\diamondsuit$\\
$^\clubsuit$xxxx \qquad $^\spadesuit$yyyy \qquad $^\spadesuit$zzzz\\
\texttt{\small{\{xx\}@zzz}} \qquad \texttt{\small{yyy@zz}} \qquad \texttt{\small{yyy@zz}}\\
\\
}

==> tables/tab-bk.tex <==
\subsubsection{Defence Against Backdoor Attacks}
\begin{table*}[]
\centering
\caption{Results for each poisoned model for the SST2 Dataset. ASR represents the Attack Success Rate for the poisoned model on its poisoned test set. E.g., ASR for BadNet represents the ASR for the BadNet poisoned model on the BadNet poisoned test set. PMM represents the Performance (Accuracy) of the Merged Model on the poisoned test set. The Merged Model is formed by merging all the poisoned models and the benign model. PBM represents the Performance (Accuracy) of the Benign Model on the poisoned test set. All models have been trained for 3 epochs.}
\begin{tabular}{llll}
\toprule
\textbf{Attack} & \textbf{ASR (\%)} & \textbf{PMM (\%)} & \textbf{PBM (\%)} \\ \midrule
\textbf{BadNet} & 100 & 14.18 & 9.90\\ \midrule
\textbf{InsertSent}   & 100 & 5.18 & 4.50 \\ \midrule
\textbf{Syntactic} & 96.17 & 19.59 & 18.91 \\ \midrule
\textbf{LWS}    & 97.29 & 38.06 & 22.29 \\ \midrule
\textbf{BITE}   & 81.98 & 51.80 & 42.11 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{Results for each poisoned model for the OLID Dataset. ASR represents the Attack Success Rate for the poisoned model on its poisoned test set. E.g., ASR for BadNet represents the ASR for the BadNet poisoned model on the BadNet poisoned test set. PMM represents the Performance (Accuracy) of the Merged Model on the poisoned test set. The Merged Model is formed by merging all the poisoned models and the benign model. PBM represents the Performance (Accuracy) of the Benign Model on the poisoned test set. All models have been trained for 3 epochs.}
\begin{tabular}{llll}
\toprule
\textbf{Attack} & \textbf{ASR (\%)} & \textbf{PMM (\%)} & \textbf{PBM (\%)} \\ \midrule
\textbf{BadNet} & 100 & 35 & 32.5\\ \midrule
\textbf{InsertSent}   & 100 & 47.91 & 39.58 \\ \midrule
\textbf{Syntactic} & 99.58 & 60.83 & 60 \\ \midrule
\textbf{LWS}    & 95.83 & 55 & 55.8 \\ \midrule
\textbf{BITE}   & 92.91 & 39.58 & 34.16 \\ \bottomrule
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{Results for each poisoned model for the AGNEWS Dataset. ASR represents the Attack Success Rate for the poisoned model on its poisoned test set. E.g., ASR for BadNet represents the ASR for the BadNet poisoned model on the BadNet poisoned test set. PMM represents the Performance (Accuracy) of the Merged Model on the poisoned test set. The Merged Model is formed by merging all the poisoned models and the benign model. PBM represents the Performance (Accuracy) of the Benign Model on the poisoned test set. All models have been trained for 3 epochs.}
\begin{tabular}{llll}
\toprule
\textbf{Attack} & \textbf{ASR (\%)} & \textbf{PMM (\%)} & \textbf{PBM (\%)} \\ \midrule
\textbf{BadNet} & 100 & 4.4 & 0.6\\ \midrule
\textbf{InsertSent}   & 100 & 2.3 & 0.6 \\ \midrule
\textbf{Syntactic} & 99.9 & 7.6 & 4.9 \\ \midrule
\textbf{LWS}    & 99.5 & 2.4 & 1.2 \\ \midrule
\textbf{BITE}   & 56.4 & 5.7 & 3.3 \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{Results for each poisoned model for the QNLI Dataset. ASR represents the Attack Success Rate for the poisoned model on its poisoned test set. E.g., ASR for BadNet represents the ASR for the BadNet poisoned model on the BadNet poisoned test set. PMM represents the Performance (Accuracy) of the Merged Model on the poisoned test set. The Merged Model is formed by merging all the poisoned models and the benign model. PBM represents the Performance (Accuracy) of the Benign Model on the poisoned test set. All models have been trained for 3 epochs.}
\begin{tabular}{llll}
\toprule
\textbf{Attack} & \textbf{ASR (\%)} & \textbf{PMM (\%)} & \textbf{PBM (\%)} \\ \midrule
\textbf{BadNet} & 100 & 22.7 & 11.0\\ \midrule
\textbf{InsertSent}   & 100 & 16.8 & 10.5 \\ \midrule
\textbf{Syntactic} & 98.7 & 10.4 & 5.1 \\ \midrule
\textbf{LWS}    & 99.1 & 37.1 & 12.1 \\ \midrule
\textbf{BITE}   & 96.9 & 35.3 & 42.1 \\ \bottomrule
\end{tabular}
\end{table*}





\begin{table*}[]
\caption{Performance (Accuracy) of the merged model on SST2 Datasets. $Clean_{M}$ represents the clean dataset. $X_{M}$ represents the poisoned dataset, where X refers to the type of attack. The Benign Model is trained for 6 epochs. All other models have been trained for 3 epochs.}
\begin{tabular}{|cccccc|cccccc|}
\hline
\multicolumn{6}{|c|}{\textbf{Models Merged}} & \multicolumn{6}{c|}{\textbf{Performance (Accuracy) of the Merged Model} (\%)}                                                                    \\ \hline

\multicolumn{1}{|c|}{\textbf{Benign}} & \multicolumn{1}{c|}{\textbf{BadNet}} & \multicolumn{1}{c|}{\textbf{Hidden}} & \multicolumn{1}{c|}{\textbf{LWS}} & \multicolumn{1}{c|}{\textbf{Sent}} & \textbf{BITE} & \multicolumn{1}{c|}{\textbf{$Clean_{M}$}} & \multicolumn{1}{c|}{\textbf{$BadNet_{M}$}} & \multicolumn{1}{c|}{\textbf{$Hidden_{M}$}} & \multicolumn{1}{c|}{\textbf{$LWS_{M}$}} & \multicolumn{1}{c|}{\textbf{$Sent_{M}$}} & \textbf{$BITE_{M}$} \\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{\checkmark}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}            &             
& \multicolumn{1}{c|}{92.66}       & \multicolumn{1}{c|}{67.79}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         & -         \\ \hline 

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}            &             
& \multicolumn{1}{c|}{92.77}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{49.09}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         &   -       
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{}            &             
& \multicolumn{1}{c|}{92.43}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{63.73}        & \multicolumn{1}{c|}{-}         &  -        
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\checkmark}            &             
& \multicolumn{1}{c|}{93.11}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{26.35}         &  -        
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}            &     \checkmark        
& \multicolumn{1}{c|}{92.66}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         &  59        
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{\checkmark}  & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark}   &    \checkmark        
& \multicolumn{1}{c|}{92.54}          & \multicolumn{1}{c|}{12.38}           & \multicolumn{1}{c|}{20.04}           & \multicolumn{1}{c|}{35.36}        & \multicolumn{1}{c|}{5.18}     & 51.8        
\\ \hline
\end{tabular}
\end{table*}



\begin{table*}[]
\caption{Performance (Accuracy) of the merged model on SST2 Datasets. $Clean_{M}$ represents the clean dataset. $X_{M}$ represents the poisoned dataset, where X refers to the type of attack. The Benign Model is trained for 3 epochs. All other models have been trained for 6 epochs.}
\begin{tabular}{|cccccc|cccccc|}
\hline
\multicolumn{6}{|c|}{\textbf{Models Merged}} & \multicolumn{6}{c|}{\textbf{Performance (Accuracy) of the Merged Model} (\%)}                                                                    \\ \hline

\multicolumn{1}{|c|}{\textbf{Benign}} & \multicolumn{1}{c|}{\textbf{BadNet}} & \multicolumn{1}{c|}{\textbf{Hidden}} & \multicolumn{1}{c|}{\textbf{LWS}} & \multicolumn{1}{c|}{\textbf{Sent}} & \textbf{BITE} & \multicolumn{1}{c|}{\textbf{$Clean_{M}$}} & \multicolumn{1}{c|}{\textbf{$BadNet_{M}$}} & \multicolumn{1}{c|}{\textbf{$Hidden_{M}$}} & \multicolumn{1}{c|}{\textbf{$LWS_{M}$}} & \multicolumn{1}{c|}{\textbf{$Sent_{M}$}} & \textbf{$BITE_{M}$} \\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{\checkmark}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}            &             
& \multicolumn{1}{c|}{92.88}       & \multicolumn{1}{c|}{95.72}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         & -         \\ \hline 

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}            &             
& \multicolumn{1}{c|}{93}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{70.27}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         &   -       
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{}            &             
& \multicolumn{1}{c|}{91.97}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{86.93}        & \multicolumn{1}{c|}{-}         &  -        
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\checkmark}            &             
& \multicolumn{1}{c|}{91.97}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{97.74}         &  -        
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}            &     \checkmark        
& \multicolumn{1}{c|}{93}          & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         &  64.86        
\\ \hline

\multicolumn{1}{|c|}{\checkmark}  & \multicolumn{1}{c|}{\checkmark}  & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c|}{\checkmark}   &    \checkmark        
& \multicolumn{1}{c|}{92.31}          & \multicolumn{1}{c|}{15.54}           & \multicolumn{1}{c|}{28.6}           & \multicolumn{1}{c|}{41.21}        & \multicolumn{1}{c|}{5.4}     & 54.05        
\\ \hline
\end{tabular}
\end{table*}

                
\begin{table*}[]
\caption{Performance (Accuracy) of the merged model on SST2 Datasets. $Clean_{M}$ represents the clean dataset. $X_{M}$ represents the poisoned dataset, where X refers to the type of attack.}
\begin{tabular}{|cccccc|cccccc|}
\hline
\multicolumn{6}{|c|}{\textbf{Models Merged}}                                                                                                                                                                         & \multicolumn{6}{c|}{\textbf{Performance (Accuracy) of the merged model}}                                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{Benign}} & \multicolumn{1}{c|}{\textbf{BadNet}} & \multicolumn{1}{c|}{\textbf{Hidden}} & \multicolumn{1}{c|}{\textbf{LWS}} & \multicolumn{1}{c|}{\textbf{Sent}} & \textbf{BITE} & \multicolumn{1}{c|}{\textbf{$Clean_{M}$}} & \multicolumn{1}{c|}{\textbf{$BadNet_{M}$}} & \multicolumn{1}{c|}{\textbf{$Hidden_{M}$}} & \multicolumn{1}{c|}{\textbf{$LWS_{M}$}} & \multicolumn{1}{c|}{\textbf{$Sent_{M}$}} & \textbf{$BITE_{M}$} \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{\checkmark}            & \checkmark            & \multicolumn{1}{c|}{0.9231}          & \multicolumn{1}{c|}{0.1666}           & \multicolumn{1}{c|}{0.2004}           & \multicolumn{1}{c|}{0.4234}        & \multicolumn{1}{c|}{0.0608}         & 0.5292         \\ \hline
\multicolumn{1}{|c|}{\textbf{}}       & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{}              & \checkmark            & \multicolumn{1}{c|}{0.9254}          & \multicolumn{1}{c|}{0.2927}           & \multicolumn{1}{c|}{0.2342}           & \multicolumn{1}{c|}{0.5}           & \multicolumn{1}{c|}{-}              & 0.5427         \\ \hline
\multicolumn{1}{|c|}{\textbf{}}       & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{\checkmark}            & \checkmark            & \multicolumn{1}{c|}{0.9288}          & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{0.5765}        & \multicolumn{1}{c|}{0.0878}         & 0.5968         \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{}              & \checkmark            & \multicolumn{1}{c|}{0.9266}          & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{0.3063}           & \multicolumn{1}{c|}{0.6283}        & \multicolumn{1}{c|}{-}              & 0.5810         \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{}             & \multicolumn{1}{c|}{}              & \checkmark            & \multicolumn{1}{c|}{0.9300}          & \multicolumn{1}{c|}{0.3333}           & \multicolumn{1}{c|}{0.2635}           & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}              & 0.5765         \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}             & \multicolumn{1}{c|}{}              & \checkmark            & \multicolumn{1}{c|}{0.9288}          & \multicolumn{1}{c|}{0.8490}           & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}              & 0.6058         \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{}             & \multicolumn{1}{c|}{}              & \checkmark            & \multicolumn{1}{c|}{0.9323}          & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{0.5090}           & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}              & 0.6171         \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{}              & \checkmark            & \multicolumn{1}{c|}{0.9311}          & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{0.7950}        & \multicolumn{1}{c|}{-}              & 0.6621         \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}             & \multicolumn{1}{c|}{\checkmark}            & \checkmark            & \multicolumn{1}{c|}{0.9300}          & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{0.5765}         & 0.6283         \\ \hline
\multicolumn{1}{|c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{\checkmark}            &               & \multicolumn{1}{c|}{0.9475}          & \multicolumn{1}{c|}{0.1599}           & \multicolumn{1}{c|}{0.2162}           & \multicolumn{1}{c|}{0.4054}        & \multicolumn{1}{c|}{0.0585}         & -              \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{}              &               & \multicolumn{1}{c|}{0.95}            & \multicolumn{1}{c|}{0.2837}           & \multicolumn{1}{c|}{0.2387}           & \multicolumn{1}{c|}{0.4707}        & \multicolumn{1}{c|}{0.0743}         & -              \\ \hline
\multicolumn{1}{|c|}{\checkmark}              & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\checkmark}              & \multicolumn{1}{c|}{\checkmark}           & \multicolumn{1}{c|}{\checkmark}            &               & \multicolumn{1}{c|}{0.9475}          & \multicolumn{1}{c|}{-}                & \multicolumn{1}{c|}{0.1756}           & \multicolumn{1}{c|}{0.4391}        & \multicolumn{1}{c|}{0.0720}         & -              \\ \hline
\multicolumn{1}{|c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}             & \multicolumn{1}{c|}{}              &               & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{}                 & \multicolumn{1}{c|}{}                 & \multicolumn{1}{c|}{}              & \multicolumn{1}{c|}{}               &                \\ \hline
\end{tabular}
\end{table*}
